On Compact Routing for the Internet

While there exist compact routing schemes designed for grids, trees, and Internet-like topologies that offer routing tables of sizes that scale logarithmically with the network size, we demonstrate in this paper that in view of recent results in compact routing research, such logarithmic scaling on Internet-like topologies is fundamentally impossible in the presence of topology dynamics or topology-independent (flat) addressing. We use analytic arguments to show that the number of routing control messages per topology change cannot scale better than linearly on Internet-like topologies. We also employ simulations to confirm that logarithmic routing table size scaling gets broken by topology-independent addressing, a cornerstone of popular locator-identifier split proposals aiming at improving routing scaling in the presence of network topology dynamics or host mobility. These pessimistic findings lead us to the conclusion that a fundamental re-examination of assumptions behind routing models and abstractions is needed in order to find a routing architecture that would be able to scale ``indefinitely.''

==> Makefile <==
ROOT=	tex

TEXSRC=	$(ROOT).tex \
	abstract.tex \
	compactrouting.tex \
	comphist.tex \
	conclusion.tex \
	hier.tex \
	introduction.tex \
	scalability.tex \
	stretch.tex \
	lis.tex \
	dynamics.tex

BIB=	bib.bib

IMAGES= 

all: $(ROOT).pdf

.SUFFIXES: .tex .dvi .ps .pdf

$(ROOT).dvi: $(TEXSRC) $(IMAGES)

MKPASS=@mkpass() { rm -f $(ROOT).dvi; $(MAKE) $(ROOT).dvi && touch $$*;}; mkpass

.pass1:
	$(MKPASS) $@

$(ROOT).bbl: .pass1 $(BIB)
	bibtex $(ROOT)

.pass2: $(ROOT).bbl
	$(MKPASS) $@

.pass3: .pass1
	$(MKPASS) $@

$(ROOT).ps: .pass3

.tex.dvi:
	latex \\nonstopmode \\input{$<} || { rm $@; exit 1; }

.dvi.ps:
	dvips -t letter -Ppdf -G0 -o $@ $<

.ps.pdf:
	ps2pdf -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true $<

clean:
	rm -f *.aux *.log *~ *.blg 
	rm -f .pass[123]
realclean: clean
	rm -f *.ps *.dvi *.pdf *.bak *.sav
	chmod -x `find . -type f`

